Making the most of small Software Engineering datasets with modern machine learning

This paper provides a starting point for Software Engineering (SE) researchers and practitioners faced with the problem of training machine learning models on small datasets. Due to the high costs associated with labeling data, in Software Engineering,there exist many small (< 1 000 samples) and medium-sized (< 100 000 samples) datasets. While deep learning has set the state of the art in many machine learning tasks, it is only recently that it has proven effective on small-sized datasets, primarily thanks to pre-training, a semi-supervised learning technique that leverages abundant unlabelled data alongside scarce labelled data.In this work, we evaluate pre-trained Transformer models on a selection of 13 smaller datasets from the SE literature, covering both,source code and natural language. Our results suggest that pre-trained Transformers are competitive and in some cases superior to previous models, especially for tasks involving natural language; whereas for source code tasks, in particular for very small datasets,traditional machine learning methods often has the edge.In addition, we experiment with several techniques that ought to aid training on small datasets, including active learning, data augmentation, soft labels, self-training and intermediate-task fine-tuning, and issue recommendations on when they are effective. We also release all the data, scripts, and most importantly pre-trained models for the community to reuse on their own datasets.

==> coherence.tex <==
\section{Code-Comment Coherence}

\def\codeberta{\textit{CodeBERTa}}

\citet{corazza-ds, corazza, corazza-we} examine the concept of code-comment coherence.
In \citep{corazza-ds} they introduce a dataset of \numprint{2883} \textit{Java} methods
along with their leading comment and whether coherence exists between the two or not (i.e. a binary label).
In a later and extended work \cite{corazza}, they 


\subsection{Methodology}
We use the \textit{CodeBERTa}\footnote{\url{https://huggingface.co/huggingface/CodeBERTa-small-v1}}, a small (6-layer)
\roberta{} model trained on the \textit{CodeSearchNet}\citep{codesearchnet} dataset.
We concatenate the comments with the corresponding methods. 


\subsection{Intermediate Task Fine-Tuning}
We try fine-tuning our pre-trained model on an intermediate task (similar to STILT \citep{stilt}).
We use some \numprint{38000} \textit{Java} methods along with comments from the \textit{CodeSearchNet}
\citep{codesearchnet} dataset. We assign half of the methods to their real comments and the other half to 
comments selected randomly. The model is now fine-tuned on the intermediate task of detecting randomly assigned comments.
Finally we fine-tune on the final task (as above).

\subsection{Results and Conclusions}
 
\setlength{\tabcolsep}{16pt} 
\begin{table}[h]
  \begin{center}
    \begin{threeparttable}
    \begin{tabular}{lccc}
      \toprule
      \textbf{Model}  &  \textbf{Acc.} & \textbf{AUC} \\
      \midrule
      \input{coherence/results/table}
      \bottomrule
    \end{tabular}
    \begin{tablenotes}
      \item[1] Single seed; value reported in \cite{corazza}
      \item[2] Average over 5 seeds; reproduction
    \end{tablenotes}
    \end{threeparttable}
  \end{center}
  \caption{Evaluation result on the comment-code coherence dataset.}
  \label{tab:coherence-results}  
\end{table}


==> readability.tex <==
\section{Readability}
A relatively small number of papers \cite{buse, posnett, dorn, scalabrino2016, scalabrino2018} examine models for automatic code readability estimation.
Most recently, \citet{scalabrino2016, scalabrino2018} compiled a dataset\footnote{\url{https://dibt.unimol.it/report/readability/}} by letting 30 Computer Science students rate
the readability of 200 methods, previously selected from well-known \textit{Java} projects. By averaging the 9 readability ratings collected in this way and comparing against
a threshold value, each method was assigned a binary readability label.
They then build a logistic regression model for code readability estimation by combining structural readability features
proposed in \citet{buse}, and \citet{dorn} with novel textual features.

\subsection{Methodology}
Again, we make use of \textit{CodeBERTa} model; unlike previous work raw code is used as input.
Since \citet{buse} show that line length is an important feature in their model, in a second experiment we
append special line length tokens (e.g. \texttt{<l1>} for short lines, up to \texttt{<l10>} for very long lines etc.) to each line in the input.

\subsection{Results and Conclusions}
The \roberta{} model is unable improve on previous work. Line length tokens seem to deteriorate performance.

\begin{table}[h]
  \begin{center}
    \input{readability/results/table}
  \end{center}
  \caption{Results for the readability task}
  \label{tab:readability-results}
\end{table}  
    


==> satd.tex <==
\section{Self-Admitted Technical Debt}

By self-admitted technical debt (SATD) we understand technical debt known to and acknowledged by the author that is often marked in code comments with
a short description of a flaw or shortcoming, often, but not always, preceded by specific keywords, such as \texttt{FIXME}, \texttt{TODO} or \texttt{HACK}.

Detection of such comments can be useful to assess software quality, aid decision-making or direct further development.

\citet{satd-orig} compiled an extensive dataset of comments classified as either a type of SATD (largely following \citep{satd-ontology}) or not from various popular \textit{Java} projects (Table \ref{tab:satd-ds});
we apply this dataset to \bert{}-like models and compare our results with existing methods.

\begin{table}[h]
  \footnotesize
  \begin{center}
    \input{satd/dataset/table}
  \end{center}
  \caption{Projects in the SATD dataset along with the number of samples mentioning self-admitted technical debt.} 
  \label{tab:satd-ds}
\end{table}

\subsection{Related Work}
For a survey on self-admitted technical debt see e.g. \citet{satd-survey}. \citet{satd-orig}, beside introducing the dataset use in this work,
also convey various SATD detection and classification experiments using traditional methods of NLP and machine learning. \citet{satd-cnn} use Convolutional
Neural Networks to detect SATD, also relying on the dataset from \citep{satd-orig}. A text-mining based approach to SATD detection can be found in \citep{satd-tm1, satd-tm2}.

\subsection{Methology}

We train our \stackobertflowshort{} in a 9 $\rightarrow$ 1 cross-project setting. That is, we use 9 out of the 10 total projects for training and evaluate on the
remaining project. Similar to what \citet{satd-orig} are doing, we preprocess the input: we remove newlines, comment delimiters (e.g. \texttt{//}, \texttt{/*}, \texttt{*/}),
\textit{HTML} fragments, \textit{JavaDoc} notation (e.g. \texttt{@param}, \texttt{@link}) and all punctuation except periods and question marks.







\subsection{Self-Training}

We attempt to use self-training (self-labelling, self-learning) \citep{self-training1, self-training2}, a very simple semi-supervised learning method.
We extract some \numprint{350000} comments from various popular \textit{Java} libraries and frameworks.
We train a classifier model on the entire original dataset. We use this model to classify the \numprint{350000} comments as either \textit{technical debt} or \textit{not technical debt}.
We only keep the roughly \textit{3900} (positive) comments classified as \textit{technical debt} and discard all other samples to avoid increasing the class imbalance already extant in the original dataset.
For each positive sample we calculate a confidence score using $C_{LC}$ (Table \ref{tab:acqfuncs}).
We take the top 5\%, and 80\% most confidently classified comments, equal to \numprint{6092} and \numprint{7880} additional comments respectively, add them to the original training set
and repeat the standard training and evaluation procedure. As can be clearly seen in figure \ref{fig:self-train}, self-training can be
used to increase recall (and possibly F1) at the cost of a reduction in precision, allowing to tune the two metrics according to task-specific needs.

\begin{figure}
    \begin{center}
        \scalebox{0.65}{\input{satd/self_train/out.pgf}}
    \end{center}
    \caption{Precision, recall and F1 under different self-training settings for the \textit{Apache Ant} project.}
    \label{fig:self-train}
\end{figure}

\subsection{Results and Conclusions}

Our model is able to outperform the \textit{CNN} model by \citet{satd-cnn}, which, to the best of our knowledge, represents the current state of the art (see Table \ref{tab:satd-results}). The dataset contains a considerable number of exact duplicates and near duplicates (those arising after preprocessing): we report results with and without removal of such duplicates.
Using self-training, we were able to achieve an even higher F1 score of 


Table \ref{tab:satd-top-loss} lists the misclassified comments with the largest loss (two false positives and two false negatives per project). Notably, false positives often contain keywords such as \texttt{FIXME}, \texttt{TODO}, or \texttt{HACK}; while this might raise questions about the quality of the dataset used, we found that only 1.2\% of the negative instances contain such keywords, compared to 6\% among positives. 

\setlength{\tabcolsep}{2pt}
\begin{table}
  \footnotesize
  \begin{center}
    \begin{threeparttable}
    \begin{tabular}{@{\extracolsep{4pt}}lcccccccccc@{}}
      \toprule
      {} & \multicolumn{4}{c}{\textbf{F1}} & \multicolumn{3}{c}{\textbf{Precision}} & \multicolumn{3}{c}{\textbf{Recall}} \\
      \cline{2-5}
      \cline{6-8}
      \cline{9-11}
      & CNN~\citep{satd-cnn}  &  NLP~\citep{satd-orig} &  Ours\tnote{1} & Ours\tnote{2} &  CNN~\citep{satd-cnn} &  Ours\tnote{1} & Ours\tnote{2} & CNN~\citep{satd-cnn} & Ours\tnote{1} & Ours\tnote{2} \\
      \midrule
      \input{satd/results/table}
      \bottomrule
    \end{tabular}
    \begin{tablenotes}
      \item[1] with duplicates
      \item[2] without duplicates
    \end{tablenotes}
    \end{threeparttable}
  \end{center}
  \caption{Comparison of macro F1, precision and recall of the different projects in the dataset. As far as our results are concerned, numbers are means over five runs, each with different seed.}
  \label{tab:satd-results}
\end{table}
\setlength{\tabcolsep}{6pt}


\begin{table}
  \footnotesize
  \begin{center}
    \begin{tabular}{ccp{12cm}}
      \toprule
      \textbf{Project}&\textbf{Error Type}&\textbf{Comment}\\
      \midrule
      \input{satd/top_loss/table}%
      \bottomrule
    \end{tabular}      
  \end{center}
   \caption{False positives and false negatives with largest loss for each project in the dataset.}
   \label{tab:satd-top-loss}
\end{table}





==> satd/results/table.tex <==
\textbf{Apache Ant} &          71.1 &  \bftab 74.8 &                 70.1 &                73.7 &         68.7 &         69.2 &         58.4 &             71.8 &            70.2 &          69.4 &         66.4 &                 64.0 &                64.9 &        62.6 &         65.5 &  \bftab 75.8 &             63.7 &            67.9 \\
\textbf{ArgoUML   } &          85.1 &         84.5 &          \bftab 85.9 &                85.4 &         84.8 &         84.9 &         81.6 &             84.4 &            83.7 &          95.0 &         95.0 &                 94.4 &         \bftab 95.2 &        95.2 &         95.1 &         95.0 &             94.9 &            95.0 \\
\textbf{Columba   } &          88.9 &         89.1 &                 89.7 &                89.9 &  \bftab 90.3 &         88.8 &         83.0 &             90.1 &            89.2 &          93.1 &         93.9 &                 91.1 &                92.9 &        91.8 &  \bftab 95.2 &         87.5 &             89.9 &            92.2 \\
\textbf{EMF       } &   \bftab 82.0 &         77.3 &                 77.9 &                72.1 &         81.9 &         81.6 &         79.3 &             76.8 &            78.0 &          66.9 &  \bftab 69.4 &                 68.1 &                69.4 &        66.4 &         68.5 &         59.4 &             64.9 &            66.2 \\
\textbf{Hibernate } &          91.3 &         92.5 &                 90.8 &                92.1 &         91.5 &         91.9 &  \bftab 93.0 &             90.6 &            88.8 &          86.1 &         85.2 &                 84.5 &                84.8 &        85.2 &         86.2 &         74.3 &             84.5 &     \bftab 86.7 \\
\textbf{JEdit     } &          74.3 &         74.7 &                 69.5 &                71.2 &         70.4 &         71.9 &  \bftab 77.3 &             74.4 &            70.4 &          72.2 &         69.5 &                 71.8 &                70.5 &        73.7 &         69.8 &         48.9 &             73.6 &     \bftab 74.4 \\
\textbf{JFreeChart} &          72.4 &         71.4 &          \bftab 78.7 &                72.6 &         75.3 &         71.1 &         68.6 &             72.2 &            66.5 &          83.9 &         58.3 &                 83.9 &                58.5 &        83.7 &         57.9 &         80.2 &      \bftab 84.9 &            60.0 \\
\textbf{JMeter    } &          89.7 &         91.9 &                 91.3 &         \bftab 92.7 &         91.9 &         92.0 &         87.3 &             86.7 &            86.3 &          84.5 &         81.5 &                 84.1 &                79.9 &        83.4 &         81.1 &         78.7 &      \bftab 86.6 &            82.5 \\
\textbf{JRuby     } &          89.9 &         91.0 &                 90.3 &                91.3 &         90.0 &  \bftab 91.7 &         80.5 &             89.3 &            89.0 &          92.4 &         93.2 &                 92.2 &                93.6 &        91.6 &         93.0 &         93.0 &             91.7 &     \bftab 94.0 \\
\textbf{SQuirrel  } &          81.6 &  \bftab 82.9 &                 82.6 &                81.1 &         82.2 &         82.4 &         79.4 &             78.7 &            81.4 &          76.9 &         78.7 &                 74.3 &                78.3 &        75.8 &  \bftab 78.7 &         69.2 &             78.7 &            76.2 \\
\midrule
\textbf{Average   } &          82.6 &  \bftab 83.0 &                 82.7 &                82.2 &         82.7 &         82.6 &         78.8 &             81.5 &            80.3 &   \bftab 82.0 &         79.1 &                 80.9 &                78.8 &        80.9 &         79.1 &         76.2 &             81.3 &            79.5 \\

==> satd/top_loss/table.tex <==
false neg. &  // Not yet ready // DataImportGlobalPreferencesTab tab = new DataImportGlobalPreferencesTab(); // return new IGlobalPreferencesPanel{[}{]} \{ tab \}; \\
false neg. &  // The following query produces a result that should be editable, but it currently isn't \\
false neg. &  // Required otherwise it gets too wide. \\
false neg. &  // Empty implementation. \\
false neg. &  // we might need to perform a DST correction \\
false neg. &  // if the method is extending something, then we have // to test if the handler is initialized... \\
false neg. &  // we basically ignore protocol. let someone report it... \\
false neg. &  //??GETRIDOFTHIS \\
false neg. &  // NOTUSED yet private JTextField filename; \\
false neg. &  /*     * NOTUSED private void initButtonMap() \{ \}     */ \\
false pos. &  // TODO move to new standard location and rewrite test to be less static \\
false pos. &  // TODO: Comments are on Element in UML 2.x \\
false pos. &  // TODO: assumes public, user pref for default visibility? //do I have to check the namespace here? (Toby) \\
false pos. &  // TODO: We just need to get someone to re{-}render a single // line of text which represents the element here, but I'm // not sure how to do that. {-} tfm // TODO: Bob replies {-} we shouldn't be interested in this // event here. The FigFeature (or its notation) should be // listen for change and the FigFeature should be update // from that. \\
false pos. &  // XXX this should be done in CollectionsModelInterpreter // but it can't trigger another invokeFeature... \\
false pos. &  /* TODO: Do we need to clone the stereotype(s)? */ \\
false pos. &  // TODO: I18N // Don't use the empty string for this or it won't show in the list \\
false pos. &  // TODO: We shouldn't need this as well as the above. \\
false pos. &  // TODO: The WFR doesn't restrict this to Classifiers {-} tfm \\
false pos. &  // Get all classifiers in our model // TODO: We need the property panels to have some reference to the // project they belong to instead of using deprecated functionality \\

==> sentiment.tex <==
\section{Sentiment Classification}

We investigate the use of \bert{}-like models for the task of sentiment classification in software engineering. That is, assigning to a sentence with content related to
software development a sentiment class (i.e. \textit{positive}, \textit{negative}, \textit{neutral}).

Building on previous work, we use the datasets compiled by \citet{senti4sd} and \citet{howfarcanwego, twodssenti} (see Table \ref{tab:sentids}). 

\begin{table}
  \begin{center}
    \input{sentiment/datasets/table}
  \end{center}
  \caption{Sentiment classification datasets considered in this work.} 
  \label{tab:sentids}
\end{table}


\subsection{Related Work}

There is vast literature on sentiment analysis and classification. For an overview see e.g. \citep{MANTYLA201816}.
Recent works on this topic include \citep{munikar2019fine, teng2016context, thongtan-phienthrakul-2019-sentiment}; notably \citep{munikar2019fine} is using a \bert{}\citep{bert} model.
\citet{howfarcanwego} investigate the performance of various sentiment analysis tools on different software-related datasets while also introducing a novel model
trained on \stackoverflow{} discussions. In a similar vein, \citet{senti4sd} use embeddings trained on a \stackoverflow{} corpus to classify \stackoverflow{} artifacts, such as questions, answers and comments and compare their method against various baselines. \citet{senticr} introduce a new sentiment analysis tool that makes use of POS tags and builds on traditional machine-learning algorithms such as Gradient Boosting Tree.

\subsection{Methology}

We compare two approaches affordable even with relatively modest computational budget: fine-tuning a run-off-the-mill pre-trained \bert{}\citep{bert} with two data and 
training a small \roberta{} \citep{roberta} model from scratch.
For the former, we fine-tune a 12-layer (base) \bert{} model pre-trained on general English text on one (\SI{147}{\mega\byte}) and two million (\SI{304}{\mega\byte}) of \stackoverflow{} comments, respectively, taken from the \textit{Stack Exchange Data Dump}\footnote{\url{https://archive.org/details/stackexchange}}.
For the latter, we train from scratch a 6-layer (small) \roberta{} model on 26.2 million \textit{StackOverflow} comments (\SI{3.6}{\giga\byte}).
We fine-tune for two epochs; from scratch training is done for five epochs. In both cases we use a maximum sequence length of 256.
Our small model, called \stackobertflow{}, is publicly available\footnote{\url{https://huggingface.co/giganticode/StackOBERTflow-comments-small-v1}}.

We train these models (after pre-training and fine-tuning) on the \stackoverflow{} sentiment classification dataset from \citet{senti4sd}, using also the same train-test split; 30\% of the training set was used as validation set.
We evaluate the models on the test set and three more datasets from \citep{twodssenti, howfarcanwego} (see Table \ref{tab:sentids})

To get a rough estimate of the effect of pre-training, we also train a randomly initialized small \roberta{} model
solely on task-specific data (i.e. the training set), see Figure \ref{fig:senti-no-pretrain}.


\subsection{Results and Conclusions}

An extensive performance comparison between our models and various baselines in given in Table \ref{tab:senti-results}.
Our results suggest that, generally, fine-tuning should be preferred over training from scratch. The fine-tuned models slightly outperformed
our from-scratch-trained model in most datasets and metrics.
Maybe more importantly fine-tuning required considerably less training time: fine-tuning took less than a day, training from scratch close to a week.
Our experiments also seem to show that as far as pre-training is concerned, relatively small amounts of data (ca. \SI{150}{\mega\byte}) are sufficient: doubling the amount
of pre-training data resulted in close to negligible improvement.

What speaks for our small model is its size: with only half the layers, training and evaluation is roughly twice as fast,
the memory footprint much smaller and performance only slightly behind a fine-tuned \bert{} model twice the size.
Thus, when carrying out a larger number of experiments, using a smaller model can speed-up progress and if no such small, pre-trained model is available,
training one from scratch can be justified.

We can also state that pre-training is essential to training \bert{}-like models: the randomly initialized model not only converges more slowly, it also has higher variance
and reaches lower peak performance (Figure \ref{fig:senti-no-pretrain}).

Finally, as can be seen in table \ref{tab:senti-top-loss}, sentences that are most confusing to the model are hard to classify even for humans.


\begin{table}
  \footnotesize
  \begin{center}
    \input{sentiment/top_loss/table}%
  \end{center}
   \caption{Sentences from the test set of the \stackoverflow{}~\citep{senti4sd} with highest loss along with predicted and actual labels and whether all raters agreed on the actual label.}
   \label{tab:senti-top-loss}
\end{table}



\begin{figure}
    \begin{center}
        \scalebox{0.7}{\input{sentiment/no_pretrain/out.pgf}}
    \end{center}
    \caption{F1 score on different sentiment classification datasets with and without pre-training. Number of optimization steps is shown on the x-axis.}
    \label{fig:senti-no-pretrain}
\end{figure}

\setlength{\tabcolsep}{2pt}
\begin{table}
  \footnotesize
  \begin{center}
    \begin{tabular}{@{\extracolsep{4pt}}llllllllll@{}}
      \toprule
       \multirow{2}{*}{\textbf{Dataset}} &  \multirow{2}{*}{\textbf{Model}} &  \multirow{2}{*}{\textbf{Acc.}} &   \multirow{2}{*}{\textbf{F1}} & \multicolumn{3}{c}{\textbf{Precision}} & \multicolumn{3}{c}{\textbf{Recall}} \\
       \cline{5-7}
       \cline{8-10}
       &   &   &   &  \textbf{Pos.} & \textbf{Neg.} & \textbf{Neu.} & \textbf{Pos.} & \textbf{Neg.} & \textbf{Neu.} \\
       \midrule
       \input{sentiment/results/table}
       \bottomrule
    \end{tabular}  
  \end{center}
  \caption{Accuracy, macro F1 and per-class precision and recall for different models and datasets. Values reported are means over five runs, each with different seed. All models were trained on the training set of the \stackoverflow{} dataset from \citet{senti4sd}.} 
  \label{tab:senti-results}
\end{table}
\setlength{\tabcolsep}{6pt}

\subsection{Soft-Labels}

We also conduct various soft-label and label-smoothing \citep{szegedy2016rethinking, muller2019does} experiments, exploiting the fact that \citet{senti4sd} release, along with the majority label, the multi-rater labels (three per sample).
From these multi-rater labels we calculate a soft-label, that is, a distribution over the three rater labels. As an example, consider the case
where one voter assigned the \textit{positive} label to a sentence, while the other two rater assigned \textit{neutral}. After majority voting,
the sentence is assigned the \textit{neutral} class.
Instead, the soft-label we calculate captures all three labels, assigning the distribution: (positive: $0.\overline{33}$, negative: $0$, neutral: $0.\overline{66}$)
to the sentence.
We train our \stackobertflowshort{} model with hard-labels, soft-labels and different degrees of label-smoothing ($\alpha$) respectively, and evaluate on all datasets (as above);
refer to Table \ref{tab:soft-labels} for a comparison of the results.

\begin{table}
  \footnotesize
  \begin{center}
    \begin{tabular}{llr@{${}\pm{}$}rr}
      \toprule
      \multirow{2}{*}{\textbf{Dataset}} &  \multirow{2}{*}{\textbf{Label Type}} &  \multicolumn{3}{c}{\textbf{F1}}\\
      \cline{3-5}
                                        &                                       &  \multicolumn{2}{c}{$\mu \pm \sigma$} & $max$ \\
      \midrule                                        
      \input{sentiment/soft_label/table}
      \bottomrule
    \end{tabular}
  \end{center}
  \caption{Macro F1 for different label types and datasets: mean, maximum and standard deviation over five runs, each with different seed. All models were trained on the training set of the \stackoverflow{} dataset from \citet{senti4sd}.}
  \label{tab:soft-labels}
\end{table}

\subsection{Active Learning}


\def\Dtest{\mathcal{D}_{test}}
\def\Dpool{\mathcal{D}_{pool}}
\def\Dseed{\mathcal{D}_{seed}}
\def\Dtop{\mathcal{D}_{top}}

The active learning experiment was carried out as follows: initially we split the training set into a seed set $\Dseed$ containing 5\% of all samples and
a pool set $\Dpool$, containing the remaining samples. We train the model on $\Dseed$, then we evaluate $\Dpool$ and the test set on this model.
Then, for each $x \in \Dpool$ we calculate a confidence score by applying an acquisition function from Table \ref{tab:acqfuncs}.
Next, we let $\Dtop$ be the $k=180$ samples with the lowest confidence score. We remove these samples from $\Dpool$ ($\Dpool = \Dpool \setminus \Dtop$)
and add them to $\Dseed$ ($\Dseed = \Dseed \cup \Dtop$). This procedure is repeated until $|\Dpool| < k$. Figure \ref{fig:act-learn} shows evaluation
results at each iteration step. Using active learning seems to result in a slightly faster convergence relative to a random baseline ($C_{rand}$).

\subsubsection*{Diversity Sampling}

Next to confidence sampling, done above, one can apply diversity sampling to avoid introducing similar samples into the pool. The process is very similar: instead
of $k$ samples, we select $c \cdot k$ samples from the pool, where $c$ determines the cluster size. We use the \textit{k}-means algorithm to cluster the $c \cdot k$ samples 
into $k$ clusters, each of size $c$. We then select a single sample from each cluster, for a total of $k$ samples. Then, we proceed as above. Figure \ref{fig:act-learn} shows evaluation results at each iteration step with a cluster size of $c=3$.

\begin{table}
  \small
  \begin{center}
    \begin{tabular}{rr@{=}l}
       & \multicolumn{2}{c}{}\\
       \toprule
       Least Confidence & $C_{LC}(x)$ & $\frac{n}{n-1}(1 - P_\theta(y^{*}_{1}|x))$ \\
       \addlinespace[0.2em]
       Margin Confidence & $C_{MC}(x)$ & $1 - (P_\theta(y^{*}_{1}|x) - P_\theta(y^{*}_{2}|x))$ \\
       \addlinespace[0.2em]       
       Ratio Confidence & $C_{RC}(x)$ & $\frac{P_\theta(y^{*}_{1}|x)}{P_\theta(y^{*}_{2}|x)}$ \\
       \addlinespace[0.2em]       
       Entropy & $C_{E}(x)$ & $-\frac{1}{log_2(n)}\sum_{i=1}^n{P_\theta(y_{i}|x)log_2(P_\theta(y_{i}|x))}$ \\
       \addlinespace[0.2em]
       Random Confidence & $C_{rand}(x)$ & $rand([0, 1])$ \\
       \bottomrule
    \end{tabular}
  \end{center}
  \caption{Acquisition functions used in our active learning experiment, adapted from \citep{humanintheloop}. $y^{*}_{1}$ and $y^{*}_{2}$ are the classes with highest and second highest probabilities, respectively; $n$ is the number of classes. All functions have range $[0, 1]$.}
  \label{tab:acqfuncs}
  
\end{table}

\begin{figure}
    \begin{center}
        \scalebox{0.65}{\input{sentiment/active_learn/out.pgf}}
    \end{center}
    \caption{F1 scores of $\Dpool$ and the test set at each iteration of the active learning process for different acquisition functions with ($c=3$) and without ($c=1$) diversity sampling.}
    \label{fig:act-learn}
\end{figure}




==> sentiment/datasets/table.tex <==
\begin{tabular}{lrrrrl}
\toprule
\textbf{Dataset} & \textbf{Negative} & \textbf{Neutral} & \textbf{Positive} & \textbf{Total} & \textbf{Usage}\\
\midrule
 \dssentiforsd{} &      1202 &     1694 &      1527 &   4423 &  Train, Test, Valid. \\
     \dsapprev{} &       130 &       25 &       186 &    341 &                 Test \\
         \dsso{} &       178 &     1191 &       131 &   1500 &                 Test \\
       \dsjira{} &       636 &        0 &       290 &    926 &                 Test \\
\bottomrule
\end{tabular}
